A Hybrid Model and Learning-Based Force Estimation Framework for Surgical Robots

Haptic feedback to the surgeon during robotic surgery would enable safer and more immersive surgeries but estimating tissue interaction forces at the tips of robotically controlled surgical instruments has proven challenging. Few existing surgical robots can measure interaction forces directly and the additional sensor may limit the life of instruments. We present a hybrid model and learning-based framework for force estimation for the Patient Side Manipulators (PSM) of a da Vinci Research Kit (dVRK). The model-based component identifies the dynamic parameters of the robot and estimates free-space joint torque, while the learning-based component compensates for environmental factors, such as the additional torque caused by trocar interaction between the PSM instrument and the patient's body wall. We evaluate our method in an abdominal phantom and achieve an error in force estimation of under 10% normalized root-mean-squared error. We show that by using a model-based method to perform dynamics identification, we reduce reliance on the training data covering the entire workspace. Although originally developed for the dVRK, the proposed method is a generalizable framework for other compliant surgical robots. The code is available at https://github.com/vu-maple-lab/dvrk_force_estimation.

==> IROS_comments.tex <==
Editor: 
 
All oral presentations will be 15 minutes; please, plan to speak for 12 minutes and allow 3 minutes for questions and answers. All oral pitch presentations will be 3 minutes, with no questions and answers, and the work will be also presented in a 2-hour interactive session based on a poster. We also solicit your presentation video clip in advance of the conference. The details will be announced later. In case of any travel difficulties, the video will be played during the session. Please contact the organizers if you wish to arrange a remote presentation instead. The final version of your manuscript must be uploaded to PaperPlaza by 31 August 2024 at 23:59 PST.

Reviewer 1: 

1, The NN consist of two linear layers with a ReLU activation layer in between. A brief explanation why the authors have used this particular design is missing. 


2, The experimental results look good, with RMSE around 2N for all force dimensions. Eq. (11) uses the spatial Jacobian. It looks to me that it makes more sense to use the dynamically consistent generalized inverse Jacobian. 


3, Clarity of most figures has to improve. The caption mentions Model Based vs. Hybrid, but by looking at the plots I guess that "troc corr" is for the Hybrid approach (in Fig. 7) and another label is used in Fig. 8 for the Hybrid approach. 
 

Reviewer 2: 
1.You mentioned “Recent learning-based model identification methods are highly dependent on training data and generalize poorly”. However, your proposed method used trocar correction network. It should be made clear that this correction is not highly dependent on the training dataset. 

2.The NRMSE and RMSE of previous methods [8, 12] have shown relatively similar results to the proposed method. (ex. In Fy, [8] is better than Hybrid.) I think you should discuss this. 

3. In Fig. 7 and Fig. 8, sometimes there is a deviation from the measured data, especially inflection points. The reason should be clearly stated. 

4.What kind of the neural network did you use? It would like to clearly state the reason for your choice since there are some types of the neural network. (Ex. DNN, CNN, RNN). 


==> table_old.tex <==
\begin{table}[]
\caption {Force Estimation Benchmark: Baselines vs. LSTM 
\protect\\ RMSE and Peak-to-Peak (PP) Values (N)}
\label{tab:RMSE} 
\begin{center}
\begin{tabular}{|l|llll|}
\hline
                & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Direct\\ Dot\\ Product\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Zero \\ Velocity \\ Baseline\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Vector \\ Search \\ Baseline\end{tabular}} & LSTM \\ \hline
Fx Classic RMSE & \multicolumn{1}{l|}{3.11}                                                           & \multicolumn{1}{l|}{1.42}                                                                 & \multicolumn{1}{l|}{1.29}                                                                 & 1.08 \\ \hline
Fx Classic PP   & \multicolumn{4}{c|}{38.09}                                                                                                                                                                                                                                                         \\ \hline
Fy Classic RMSE & \multicolumn{1}{l|}{3.93}                                                           & \multicolumn{1}{l|}{1.57}                                                                 & \multicolumn{1}{l|}{1.43}                                                                 & 0.90 \\ \hline
Fy Classic PP   & \multicolumn{4}{c|}{35.44}                                                                                                                                                                                                                                                         \\ \hline
Fz Classic RMSE & \multicolumn{1}{l|}{1.25}                                                           & \multicolumn{1}{l|}{1.523}                                                                & \multicolumn{1}{l|}{1.49}                                                                 & 0.89 \\ \hline
Fz Classic PP   & \multicolumn{4}{c|}{20.22}                                                                                                                                                                                                                                                         \\ \hline
Fx Si RMSE      & \multicolumn{1}{l|}{13.73}                                                          & \multicolumn{1}{l|}{11.88}                                                                & \multicolumn{1}{l|}{9.68}                                                                 & 2.47 \\ \hline
Fx Si PP        & \multicolumn{4}{c|}{36.33}                                                                                                                                                                                                                                                         \\ \hline
Fy Si RMSE      & \multicolumn{1}{l|}{24.52}                                                          & \multicolumn{1}{l|}{11.20}                                                                & \multicolumn{1}{l|}{9.67}                                                                 & 2.41 \\ \hline
Fy Si PP        & \multicolumn{4}{c|}{32.39}                                                                                                                                                                                                                                                         \\ \hline
Fz Si RMSE      & \multicolumn{1}{l|}{15.56}                                                          & \multicolumn{1}{l|}{3.00}                                                                 & \multicolumn{1}{l|}{2.94}                                                                 & 1.60 \\ \hline
Fz Si PP        & \multicolumn{4}{c|}{55.69}                                                                                                                                                                                                                                                         \\ \hline
\end{tabular}
\end{center}
\end{table}
